Analysing Mixed Initiatives and Search Strategies during Conversational Search

Information seeking conversations between users and Conversational Search Agents (CSAs) consist of multiple turns of interaction. While users initiate a search session, ideally a CSA should sometimes take the lead in the conversation by obtaining feedback from the user by offering query suggestions or asking for query clarifications i.e. mixed initiative. This creates the potential for more engaging conversational searches, but substantially increases the complexity of modelling and evaluating such scenarios due to the large interaction space coupled with the trade-offs between the costs and benefits of the different interactions. In this paper, we present a model for conversational search -- from which we instantiate different observed conversational search strategies, where the agent elicits: (i) Feedback-First, or (ii) Feedback-After. Using 49 TREC WebTrack Topics, we performed an analysis comparing how well these different strategies combine with different mixed initiative approaches: (i) Query Suggestions vs. (ii) Query Clarifications. Our analysis reveals that there is no superior or dominant combination, instead it shows that query clarifications are better when asked first, while query suggestions are better when asked after presenting results. We also show that the best strategy and approach depends on the trade-offs between the relative costs between querying and giving feedback, the performance of the initial query, the number of assessments per query, and the total amount of gain required. While this work highlights the complexities and challenges involved in analyzing CSAs, it provides the foundations for evaluating conversational strategies and conversational search agents in batch/offline settings.

==> 4.5_costs.tex <==
In this section, we aim to provide an estimate of various actions that a user can take in a conversation. To do so, we run multiple crowdsourcing tasks where we simulate a text-based conversation and measure the time that it takes for the user to react to different kinds of responses that the system generates. In particular, we measure the follow:
\begin{itemize}
    \item query time;
    \item snippet assessment time;
    \item document assessment time;
    \item providing feedback time.
\end{itemize}

\partitle{Task Setup.} We designed four crowdsourcing tasks (HITs) on Amazon Mechanical Turk\footnote{\url{http://mturk.com}}. In all of our tasks, we first showed the user the search topic description. We selected a total of five search topics from the TREC Web Track~\cite{DBLP:conf/trec/ClarkeCS09,DBLP:conf/trec/ClarkeCS10}. Our choice of topic was based on their difficulty and type (informational vs.~navigational and faceted vs.~ambiguous), aiming to cover a wide spectrum of search tasks in the study. Each search session starts with a query from the user. 
Figure~\ref{fig:mturk_screenshots} shows different stages of our task.
Once the user clicks the Search button, we show a result to them, as seen in Figure~\ref{fig:mturk_screenshots_snippet}. We introduced and described three levels of \textit{usefulness} to the workers, namely, useful, maybe useful, useless. As soon as the worker assesses one snippet (or document), we show the next snippet (or document). We repeat this process for five consecutive results, assuming that a user is willing to read and assess five documents ($A=5$). After assessing the fifth result, depending on the task setup, we instructed the workers to do the following:
\begin{itemize}
    \item reformulate their queries, aiming to improve the search;
    \item read and answer a clarifying question, as shown in Figure~\ref{fig:mturk_screenshots_qa}.
\end{itemize}
Out clarifying question pane design is inspired by the design of Bing.com~\citet{DBLP:conf/www/ZamaniDCBL20}. In addition, we always included a ``Not interested'' since the workers did not have the option of ignoring the question. Therefore, we instructed them to select the ``Not interested'' answer when they did not find the question relevant, or they did not find any relevant answers.
The would assess another five results after taking the actions above. Depending on the task setup, each HIT led to 20 result assessments, 1 or 4 queries, and 3 answers. Result assessment was done in two different levels:
\begin{itemize}
    \item \textbf{Snippet:} the worker would read and assess a snippet, similar to Figure~\ref{fig:mturk_screenshots_snippet};
    \item \textbf{Document:} the worker would click on a link to view a full web page and assess it.
\end{itemize}

\begin{figure}
    \centering
    \subfloat[Sample Snippet]{\includegraphics[width=\columnwidth]{figure/sample_snippet.png} \label{fig:mturk_screenshots_snippet}}
    
    \subfloat[Sample Question and Answers]{\includegraphics[width=\columnwidth]{figure/sample_question.png} \label{fig:mturk_screenshots_qa}}
    \caption{Sample result snippet and question pane used in our crowdsourcing tasks.}
    \label{fig:mturk_screenshots}
\end{figure}

\partitle{Quality Check.}
We limited the task to the workers residing in the U.S., with a total approval rate of over 98\% and 5000 total completed tasks. In addition, we included three obviously irrelevant results in each HIT and discarded a submission if those documents were assessed wrongly. Moreover, we launched the HITs sequentially and did not allow workers that took part in a previous HIT to complete a task, because the search topics were the same in all the HITs.

\partitle{Results.}
Here we present the results of the crowdsourcing. Table~\ref{tab:crowd_summary} lists a summary of the data we have collected. We provide the mean, standard deviation, and median values of the times workers spent for each type of action in Table~\ref{tab:cost_actions}. As we see, similar to previous work \cite{}, the cost of querying is much more than the cost of assessing a snippet or a full web page. What is interesting in this case is the cost of providing feedback to the agent. As we see in the table, the mean cost of providing feedback is 8.33 seconds, which is slightly higher than assessing a snippet, but half of the price of assessing a full web page. Also, it is worth mentioning that the cost of providing feedback is nearly a third of the cost of issuing a query. Moreover in Figure~\ref{fig:q_vs_rf_index}, we compare the cost of issuing a query and providing feedback in a session. The figure compares the mean cost of the two at different stages of a session (e.g., whether it is the first query or the third). We see that that the cost of both actions drops as the users get more familiar with the topic and gain more domain knowledge by assessing results. However, interestingly we see that the cost of providing feedback keeps dropping as the session goes on, whereas the cost of issuing a query goes up after three rounds. This suggests, that acquiring more domain knowledge and getting more familiar with the system leads to less time spent on both actions, but in long sessions, where the users may have exhausted all their options as queries, suggestions for feedback from the system could be more welcomed. 

\begin{table}[]
    \centering
    \caption{Summary of the collected data.}
    \begin{tabular}{ll}
        \toprule
         \# search topics & 5 \\
         \# question answer pairs & 15 \\ 
         \# search results & 100 \\
         \midrule
         \# submitted queries &     144  \\
         \# snippet assessments  &     1,280 \\
         \# web page assessments &   1,000  \\
         \# provided feedbacks & 268 \\
         \midrule
         \# workers & 81 \\
         mean query per worker & 2.72 \\
         mean snippet assessment per worker & 26.67 \\
         mean web page assessment per worker & 23.81 \\
         mean feedback per worker & 4.31 \\
         \bottomrule
    \end{tabular}
    \label{tab:crowd_summary}
\end{table}

\begin{table}[]
    \centering
    \caption{Time spend for each action by users. The differences between all the pairs are statistically significant (ttest, $p < 0.05$)}
    \begin{tabular}{lllll}
        \toprule
         &          query   & snippet   & document  & clarifying question \\
         \midrule
         mean &     29.33   &  6.26     & 16.96     & 8.33 \\
         std  &     26.46   & 12.74     & 23.38     & 9.35 \\
         median &   22.59   & 3.63      & 10.22     & 5.77 \\
         \bottomrule
    \end{tabular}
    \label{tab:cost_actions}
\end{table}
